Static Application-Level Race Detection in STM Haskell using Contracts

Writing concurrent programs is a hard task, even when using high-level synchronization primitives such as transactional memories together with a functional language with well-controlled side-effects such as Haskell, because the interferences generated by the processes to each other can occur at different levels and in a very subtle way. The problem occurs when a thread leaves or exposes the shared data in an inconsistent state with respect to the application logic or the real meaning of the data. In this paper, we propose to associate contracts to transactions and we define a program transformation that makes it possible to extend static contract checking in the context of STM Haskell. As a result, we are able to check statically that each transaction of a STM Haskell program handles the shared data in a such way that a given consistency property, expressed in the form of a user-defined boolean function, is preserved. This ensures that bad interference will not occur during the execution of the concurrent program.

==> eptcsdata.tex <==
\providecommand{\firstpage}{115}
\providecommand{\publicationstatus}{N. Yoshida, W. Vanderbauwhede (Eds.): Programming Language\\ Approaches to Concurrency- and Communication-cEntric\\Software 2013 (PLACES'13)\\
EPTCS 137, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.137.10}{10.4204/EPTCS.137.10}}
\pdfoutput=1

